Oxide: The Essence of Rust

Rust claims to advance industrial programming by bridging the gap between low-level systems programming and high-level application programming. At the heart of the argument that this enables programmers to build more reliable and efficient software is the borrow checker - a novel approach to ownership that aims to balance type system expressivity with usability. And yet, to date there is no core type system that captures Rust's notion of ownership and borrowing, and hence no foundation for research on Rust to build upon. In this work, we set out to capture the essence of this model of ownership by developing a type systems account of Rust's borrow checker. We present Oxide, a formalized programming language close to source-level Rust (but with fully-annotated types). This presentation takes a new view of lifetimes as an approximation of the provenances of references, and our type system is able to automatically compute this information through a substructural typing judgment. We provide the first syntactic proof of type safety for borrow checking using progress and preservation. Oxide is a simpler formulation of borrow checking - including recent features such as non-lexical lifetimes - that we hope researchers will be able to use as the basis for work on Rust.

==> acks.tex <==
\begin{acks}
  This material is based upon work supported in part by the National Science
  Foundation under grants CCF-1453796 and CCF-1618732, and an NSF Graduate
  Research Fellowship (GRFP) for Aaron Weiss. This work is also supported in
  part by the European Research Council under ERC Starting Grant SECOMP
  (715753). Any opinions, findings, and conclusions or recommendations expressed
  in this material are those of the author and do not necessarily reflect the
  views of the National Science Foundation nor the European Research Council.
\end{acks}

==> comparison.tex <==
To show that \lang is a faithful formal model for the (core) Rust borrow
checker, we work through a number of example programs in Rust, and their
corresponding form in \lang. Then, in \Sec{sec:tested-semantics}, we describe a
prototype type-checker for \lang and how we've used it to test our semantics
against the official borrow checker. Finally, in \Sec{sec:polonius}, we draw
connections between \lang and Polonius, a new streamlined implementation of
Rust's borrow checker using techniques from logic programming.

\subsection{Liveness}

One of the primary goals of Rust's borrow checker is to statically ensure that
there are no use-after-free errors for references since they are a common class
of bugs and even security vulnerabilities when doing systems programming in C.
To see how it works, we'll look at a small example:

\begin{rustbk}
  let msg = {
    let m = ("Howdy", "Pals");
    &m.0 // ERROR: m.0 does not live long enough
  };
  msg
\end{rustbk}

In the block spanning lines 1--4, we declare a tuple of one element on line 2,
and then create a reference to it on line 3. Since Rust is largely an
expression-based (rather than statement-based) language, when we evalute this
block, it will return the value we get from \rusti{&m.0}. However, after doing
so, \rusti{m} drops out of scope, and since it is on the stack, it is then
necessarily destroyed. If this program was allowed, we would then have a dead
pointer \emph{forward} on the stack, which would be very bad. Fortunately,
Rust's borrow checker detects this, and instead reports an error --- protecting
us from our mistake! Let's look at how the same program would work in \lang:

\begin{rustbk}
  // $\oxvarctx_0 = \oxemptyctx$
  letprov<'msg, 'm> {
    // $\oxvarctx_1 = \oxloanctxentry{\texttt{'msg}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'m}}{\{\}}$
    let msg: &'msg @\oximm@ String = {
      // $\oxvarctx_2 = \oxvarctx_1$
      let m: (String, String) = ("Howdy", "Pals");
      // $\oxvarctx_3 = \oxvarctx_2 \oxcomma \oxvarctxentry{\texttt{m}}{\oxtprod{\texttt{String}, \texttt{String}}}$
      &'m @\oximm@ m.0 // ERROR. $\oxtype = \oxtref{\texttt{'m}}{\oximm}{\texttt{String}}$
      // $\oxvarctx_4 = \oxloanctxentry{\texttt{'msg}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'m}}{\oxset{\oxloanpkg{\oximm}{\oxproj{\texttt{m}}{0}}}}$
    }; // $\texttt{'m}$ is no longer valid at this point.
    msg
  }
\end{rustbk}

To translate to \lang, we again made the usual set of changes --- annotating
bindings with types, and adding explicit $\oxkey{letprov}$ and $\oximm$
qualifiers. To aid comprehension, we also added comments that describe the state
of the stack typing $\oxvarctx$ while type-checking the program. Like the Rust
version, the \lang version statically produces an error, but to understand why
we must cover a few facts. First, recall that our rule for let binding
(\oxname{T-Let}) removes bound variables from the environments at the end of the
binding (seen on line 9). Further, note that the type we derive for
$\oxref{\rusti{'m}}{\oximm}{\oxproj{m}{0}}$ has provenance \rusti{'m} mapped to
$\oxset{\oxloanpkg{\oximm}{\oxproj{m}{0}}}$. Then, since type well-formedness
requires that the places present in the loan sets for each provenance be bound,
we are unable to prove that the type of the expression being bound for
\rusti{msg} is valid. That is,
$\oxtypevalidity{\oxemptyctx}{\oxemptyctx}{\oxvarctx_4}
{\oxtref{\texttt{'m}}{\oximm}{\texttt{String}}}$ does not hold.


\subsection{Conditional Control Flow}

It is also important for the borrow checker to be able to deal appropriately
with conditional control flow. As mentioned in \Sec{sec:formalizing}, it is
essential to treat conditional loans as live in order to have a sound analysis.
To see how \lang handles conditional control flow, we will look at two examples
in Rust and \lang --- one that type-checks and one that does not. We'll start
with the former:

\begin{rustbk}
  struct Point(u32, u32);
  let mut pt: Point = Point(3, 2);
  if cond {
      let x = &mut pt.0;
      *x = 4;
  } else {
      let p = &mut pt;
      (*p).1 = 5;
  }
\end{rustbk}

In Rust, we declare a mutable binding \rusti{pt} to a \rusti{Point} value.
Then, we branch on an unknown boolean variable \rusti{cond}, and in one case
uniquely borrow the first projection of \rusti{pt} before assigning it a new
value. In the other case, we uniquely borrow the whole of \rusti{pt}, and then
mutate its second projection through this reference. Since Rust identifies that
only one of these will happen in any program, it is okay for the two unique
references to refer to overlapping parts of memory. The program is largely the
same in \lang (though we have again included comments marking the state of the
environments during type-checking):

\begin{rustbk}
  struct Point(u32, u32);
  // $\oxvarctx_0 = \oxemptyctx$
  letprov<'a, 'b> {
    // $\oxvarctx_1 = \oxloanctxentry{\texttt{'a}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'b}}{\{\}}$
    let pt: Point = Point(3, 2);
    // $\oxvarctx_2 = \oxvarctx_1 \oxcomma \oxvarctxentry{\texttt{pt}}{\texttt{Point}}$
    if cond { // $\oxvarctx_3 = \oxvarctx_2$
        let x: &'a @\oxmut@ u32 = &'a @\oxmut@ pt.0;
        // $\oxvarctx_4 = \oxloanctxentry{\texttt{'a}}{\oxset{\oxloanpkg{\oxmut}{\texttt{pt.0}}}} \oxcomma \oxloanctxentry{\texttt{'b}}{\{\}} \oxcomma \oxvarctxentry{\texttt{pt}}{\texttt{Point}} \oxcomma \oxvarctxentry{\texttt{x}}{\oxtref{\texttt{'a}}{\oxmut}{\oxtnum}}$
        *x = 4;
        // $\oxvarctx_5 = \oxvarctx_4$
        () // $\oxvarctx_6 = \oxvarctx_2$
    } else { // $\oxvarctx_7 = \oxvarctx_2$
        let p: &'b @\oxmut@ Point = &'b @\oxmut@ pt;
        // $\oxvarctx_8 = \oxloanctxentry{\texttt{'a}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'b}}{\oxset{\oxloanpkg{\oxmut}{\texttt{pt}}}} \oxcomma \oxvarctxentry{\texttt{pt}}{\texttt{Point}} \oxcomma \oxvarctxentry{\texttt{p}}{\oxtref{\texttt{'b}}{\oxmut}{\texttt{Point}}}$
        (*p).1 = 5;
        // $\oxvarctx_9 = \oxvarctx_8$
        () // $\oxvarctx_{10} = \oxvarctx_2$
    } // $\oxvarctx_{11} = (\oxvarctx_{10} \oxintersect \oxvarctx_6) = \oxvarctx_2$
  }
\end{rustbk}

As usual, \rusti{mut} has been replaced with the more appropriate $\oxmut$. We
can now see more formally how this example type-checks. In particular, when we
get to the branch on line 7, according to \oxname{T-Branch}, we check the type
of each side of the branch under the same environment $\oxvarctx_2$ (visible in
the annotations on lines 8 and 16). Since they have the same input environment,
they are each able to create their own unique reference to parts of \rusti{pt}
(lines 9 and 17). Then, the bindings to \rusti{x} and \rusti{p} both end at the
end of their respective branch before returning unit (lines 13 and 21). This
means that when we union the \emph{output} environments of each branch on
line 21, we get exactly their input environments $\oxvarctx_2$, meaning that the
loans in each branch have necessarily ended.

However, it's also possible for loans to outlive the scope they are created in.
We will explore this kind of situation in our next example:

\begin{rustbkl}
  let mut m: u32 = 6;
  let mut n: u32 = 5;
  let x: &u32 = &n;
  if false {
    x = &m;
  }
  &mut m; // ERROR: cannot borrow m mutably while already borrowed
  ... // additional code using x
\end{rustbkl}

In this example, we declare two mutable bindings \rusti{m} and \rusti{n} on
lines 1 and 2. Then, on line 3, we create a shared reference to \rusti{n} and
bind it to \rusti{x}. On line 4, we branch, and assign to \rusti{x} a shared
reference to \rusti{m} instead. Then, after the branch ends, we try to mutably
borrow \rusti{m}. Even though we can see that the branch is dead code (since the
condition is always \rusti{false}), the borrow checker will not inspect the
value and will instead give us an error saying that we cannot borrow \rusti{m}
mutably twice. The program is again similar in \lang (and again annotated with
environment $\oxvarctx$):

\begin{rustbkl}
  letprov<'a, 'b, 'c> {
    // $\oxvarctx_0 = \oxloanctxentry{\texttt{'a}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'b}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'c}}{\{\}}$
    let mut m: u32 = 6;
    // $\oxvarctx_1 = \oxvarctx_0 \oxcomma \oxvarctxentry{\texttt{m}}{\oxtnum} $
    let mut n: u32 = 5;
    // $\oxvarctx_2 = \oxvarctx_1 \oxcomma \oxvarctxentry{\texttt{n}}{\oxtnum} $
    let x: &'a @\oximm@ u32 = &'a @\oximm@ n;
    // $\oxvarctx_3 = \oxloanctxentry{\texttt{'a}}{\oxset{\oxloanpkg{\oximm}{\texttt{n}}}} \oxcomma \oxloanctxentry{\texttt{'b}}{\{\}} \oxcomma \oxloanctxentry{\texttt{'c}}{\{\}} \oxcomma \oxvarctxentry{\texttt{m}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{n}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{x}}{\oxtref{\texttt{'a}}{\oximm}{\oxtnum}}$
    if false { // $\oxvarctx_4 = \oxvarctx_3$
      x := &'b @\oximm@ m;
      // $\oxvarctx_5 = \oxloanctxentry{\texttt{'a}}{\oxset{\oxloanpkg{\oximm}{\texttt{m}}}} \oxcomma \oxloanctxentry{\texttt{'b}}{\oxset{\oxloanpkg{\oximm}{\texttt{m}}}} \oxcomma \oxloanctxentry{\texttt{'c}}{\{\}} \oxcomma \oxvarctxentry{\texttt{m}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{n}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{x}}{\oxtref{\texttt{'a}}{\oximm}{\oxtnum}}$
      () // $\oxvarctx_6 = \oxvarctx_5$
    } else { // $\oxvarctx_7 = \oxvarctx_3$
      () // $\oxvarctx_8 = \oxvarctx_7$
    } // $\oxvarctx_9 = \oxvarctx_6 \oxintersect \oxvarctx_8 = $
      // $\oxloanctxentry{\texttt{'a}}{\oxset{\oxloanpkg{\oximm}{\texttt{m}} \oxcomma \oxloanpkg{\oximm}{\texttt{n}}}} \oxcomma \oxloanctxentry{\texttt{'b}}{\oxset{\oxloanpkg{\oximm}{\texttt{m}}}} \oxcomma \oxloanctxentry{\texttt{'c}}{\{\}} \oxcomma \oxvarctxentry{\texttt{m}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{n}}{\oxtnum} \oxcomma \oxvarctxentry{\texttt{x}}{\oxtref{\texttt{'a}}{\oximm}{\oxtnum}}$
    &'c @\oxmut@ m; // ERROR: cannot borrow m uniquely while already borrowed
    ... // additional code using x
  }
\end{rustbkl}

Now, using the \lang version of the example, we can explain more formally why
the program fails to type-check. On line 7, when we borrow from \rusti{n}, we
produce a reference of type $\oxtref{\rusti{'a}}{\oximm}{\oxtnum}$ and add it to
our stack typing as the type of \rusti{x} (line 7). Then, in the first half of
the branch, we assign to \rusti{x} a shared reference to \rusti{m} (line 11).
According to \oxname{OL-OverrideLocalProvenances} (via \oxname{T-Assign}), this
will cause us to replace the loans associated with \rusti{'a} with the loans
associated with \rusti{'b} (namely $\oxset{\oxloanpkg{\oximm}{\texttt{m}}}$),
but in the other side of the branch, we don't change \rusti{'a} and so it
remains the same (lines 12 and 18 respectively). When we exit the branch, in
\oxname{T-Branch}, we will combine the two stack typings from each side,
resulting in the unification of the loan sets associated with each provenance in
each side of the branch. The result (as seen on line 19) is that \rusti{'a} is
$\oxset{\oxloanpkg{\oximm}{\texttt{m}} \oxcomma
  \oxloanpkg{\oximm}{\texttt{n}}}$. Thus, when we attempt to derive ownership
safety in \oxname{T-Borrow} for the borrow expression on line 21, we find an
overlapping shared loan against \rusti{m} in the loan set for \rusti{'a} and
yield an error.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "essence"
%%% fill-column: 80
%%% End:


==> oxide/aliasing-inv.tex <==
\begin{lstlisting}
$\oxwellaliasedframe{\oxtvarctx}{\oxvarctx}{\oxstore}$ =
  $\forall \oxplace \in \oxdomain{\oxvarctx} $. $
    \oxmusafety{\oxtvarctx}{\oxkontctx}{\oxvarctx}{\oximm}{\oxplace}{
      \oxset{\overline{\oxloan}}
    } \implies$
    $\oxstore = \oxnewframe{\oxstore_1}{\oxnewframe{\oxstackframe_\oxplace}{\oxstore_2}}$ $\wedge$ $\oxplace \in \oxstackframe_\oxplace \wedge \oxplace \not \in \oxstore_2$ $\wedge$ $\oxvarctx(\oxplace) = \oxtref{\oxcprov}{\oxmuta}{\oxxitype_1}$
    $\oxstackframe_\oxplace(\oxplace) = \oxpt{\oxplace_p} \vee
      \oxstackframe_\oxplace(\oxplace) = \oxindexptr{\oxplace_p}{\oxnum} \vee
      \oxstackframe_\oxplace(\oxplace) = \oxsliceptr{\oxplace_p}{\oxnum_1}{\oxnum_2}
      \implies$
      $\forall \oxplace^\prime \mapsto v^\prime \in \oxnewframe{\oxstackframe_\oxplace}{\oxstore_2}$. $
         \oxmusafety{\oxtvarctx}{\oxkontctx}{\oxvarctx}{\oximm}{\oxplace^\prime}{
          \oxset{\overline{\oxloan}}
        }
       \implies$
        $(v^\prime = \oxptr{\oxplace_p^\prime} \vee
        v^\prime =
        \oxindexptr{\oxplace_p^\prime}{\oxnum^\prime} \vee
        v^\prime =
        \oxsliceptr{\oxplace_p^\prime}{\oxnum_1^\prime}{\oxnum_2^\prime})$ $\wedge$ $\oxvarctx(\oxplace^\prime) = \oxtref{\oxcprov^\prime}{\oxmuta^\prime}{\oxxitype_2}$
           $\wedge$ $\oxplace_p^\prime \in \oxdomain{\oxnewframe{\oxstackframe_\oxplace}{\oxstore_2}}$ $\wedge$ $(\oxmuta = \oxmut \vee \oxmuta^\prime = \oxmut)
           \implies \oxrelevant{\oxplace_p^\prime}{\oxplace_p}$
\end{lstlisting}


==> oxide/compute-places-typ.tex <==
\begin{lstlisting}
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ $\oxbasetype$ = $
  \oxvarctxentry{\oxplace}{\oxbasetype}$
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ $\oxtvar$ = $
  \oxvarctxentry{\oxplace}{\oxtvar}$
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ ($\oxtref{\oxprov}{\oxmuta}{
    \oxtype
  }$) = $\oxvarctxentry{\oxplace}{\oxtref{\oxprov}{\oxmuta}{\oxtype}}$
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ ($\oxtfun{
    \overline{\oxprov} \oxcomma \overline{\oxtvar}
  }{\overline{\oxtype_a}}{\oxtype_r}{\oxvarctx}$) = $
  \oxvarctxentry{\oxplace}{
    \oxtfun{
      \overline{\oxprov} \oxcomma \overline{\oxtvar}
    }{\overline{\oxtype_a}}{\oxtype_r}{\oxvarctx}
  }$
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ $\oxtarr{\oxtype}{\oxnum}$ = $
  \oxvarctxentry{\oxplace}{\oxtarr{\oxtype}{\oxnum}}
  $
  $\texttt{places-typ}_{\,\oxglobalctx}$ $\oxplace$ $\oxtprod{\oxtype_0 \oxdotsc
    \oxtype_n}$ =
      $\oxvarctxentry{\oxplace}{\oxtprod{\oxtype_0 \oxdotsc \oxtype_n}} \oxcomma$ ($
  \texttt{places-typ}_{\,\oxglobalctx}$ $\oxproj{\oxplace}{0}$ $\oxtype_0$)$
  \oxcomma$ $\oxdots\oxcomma$ ($
  \texttt{places-typ}_{\,\oxglobalctx}$ $\oxproj{\oxplace}{n}$ $\oxtype_n$)
\end{lstlisting}

==> oxide/compute-places-val.tex <==
\begin{lstlisting}
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxunit$ = $
  \oxstoreentry{\oxplace}{\oxunit}$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxnum$ = $
  \oxstoreentry{\oxplace}{\oxnum}$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxtrue$ = $
  \oxstoreentry{\oxplace}{\oxtrue}$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxfalse$ = $
  \oxstoreentry{\oxplace}{\oxfalse}$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxptr{\oxcprov}{\oxmuta}{
    \oxplace^\prime
  }$ = $\oxstoreentry{\oxplace}{\oxptr{\oxcprov}{\oxmuta}{\oxplace^\prime}}$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxindexptr{
    \oxplace^\prime
  }{\oxnum}$ = $\oxstoreentry{\oxplace}{
    \oxindexptr{\oxplace^\prime}{\oxnum}
  }$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxsliceptr{\oxcprov}{\oxmuta}{
    \oxplace^\prime
  }{\oxnum_1}{\oxnum_2}$ = $\oxstoreentry{\oxplace}{
    \oxsliceptr{\oxplace^\prime}{\oxnum_1}{\oxnum_2}
  }$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxclosureval{\oxstackframe}{
    \overline{\oxcprov} \oxcomma \overline{\oxtvar}
  }{\overline{\oxascribe{\oxid}{\oxtype}}}{\oxtype_r}{\oxexpr}$ =
      $\oxstoreentry{\oxplace}{
    \oxclosureval{\oxstackframe}{
      \overline{\oxcprov} \oxcomma \overline{\oxtvar}
    }{\overline{\oxascribe{\oxid}{\oxtype}}}{\oxtype_r}{\oxexpr}
  }$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxarr{
    \oxvalue_0 \oxdotsc \oxvalue_n
  }$ = $\oxstoreentry{\oxplace}{
    \oxarr{\oxvalue_0 \oxdotsc \oxvalue_n}
  }$
  $\texttt{places-val}_{\,\oxglobalctx}$ $\oxplace$ $\oxprod{
    \oxvalue_0 \oxdotsc \oxvalue_n
  }$ =
      $\oxstoreentry{\oxplace}{
    \oxprod{\oxshapehole_0 \oxdotsc \oxshapehole_n}
  }\oxcomma$  ($
  \texttt{places-val}_{\,\oxglobalctx}$ $\oxproj{\oxplace}{0}$ $\oxvalue_0$)$
  \oxcomma$ $\oxdots\oxcomma$ ($\texttt{places-val}_{\,\oxglobalctx}$ $\oxproj{\oxplace}{n}$ $
  \oxvalue_n$)
\end{lstlisting}


==> oxide/compute-value.tex <==
\begin{lstlisting}
  $\oxstore(\oxpathcons{\oxid}{\oxpath})$ = $\texttt{value}$ $
  \oxstore(\oxid)$ $\oxpath$
  $\texttt{value}$ $\oxvalue$ $\oxemptypath$ = $\oxvalue$
  $\texttt{value}$ $\oxprod{\oxvalue_1 \oxdotsc \oxvalue_i \oxdotsc \oxvalue_n}
  $ $\oxpathcons{i}{\oxpath}$ = $\texttt{value}$ $\oxvalue_i$ $\oxpath$
\end{lstlisting}

==> oxide/env-minus.tex <==
\begin{lstlisting}
  $\oxemptyctx \oxspace \oxenvminus\oxspace \oxid$ = $\oxemptyctx$
  $(\oxnewframe{\oxvarctx}{\oxemptyctx}) \oxspace \oxenvminus \oxspace \oxid$ = $\oxnewframe{\oxvarctx \oxspace \oxenvminus\oxspace \oxid}{\oxemptyctx}$
  $(\oxextendctx{\oxvarctx}{\oxvarctxentry{\oxid^\prime}{\oxtype}}) \oxspace \oxenvminus\oxspace \oxid$ = $
  \begin{cases}
    \oxvarctx \oxspace \oxenvminus\oxspace \oxid & \oxid = \oxid^\prime\\
    \oxextendctx{(\oxvarctx \oxspace \oxenvminus\oxspace \oxid)}{\oxvarctxentry{\oxid^\prime}{\oxtype}} & \oxid \neq \oxid^\prime
  \end{cases}$
  $\oxextendctx{\oxvarctx}{\oxloanctxentry{\oxcprov}{\oxset{\overline{\oxloan}}}}) \oxspace \oxenvminus\oxspace \oxid$ = $
  \begin{cases}
    \oxextendctx{(\oxvarctx \oxspace \oxenvminus\oxspace \oxid)}{\oxloanctxentry{\oxcprov}{\oxset{\overline{\oxloan}}}} &
    \oxforall \oxloan \in \oxset{\overline{\oxloan}}. \;
    \oxrootof{\oxloan} \neq \oxid \wedge
    (\oxcprov \not\in \oxvarctx(\oxid) \vee
    \exists \oxtype \in \oxcodomain{\oxvarctx^\prime}. \; \oxcprov \in \oxtype)
    \\
    \oxvarctx \oxspace \oxenvminus\oxspace \oxid & \texttt{else}
  \end{cases}$
\end{lstlisting}

==> oxide/loanctx-minus.tex <==
\begin{lstlisting}
$\oxvarctx - \oxplaceexpr = \oxvarctx^\prime$
  where $\oxvarctx^\prime = \oxset{
    \oxloanctxentry{\oxcprov}{\oxset{\overline{\oxloan}}} \in \oxvarctx $ | $
    \forall \oxloanpkg{\oxmuta}{\oxplaceexpr_\oxloan} \in \oxset{\overline{\oxloan}}. \;
    \oxplaceexpr \textrm{ is not a prefix of } \oxplaceexpr_\oxloan
  }$
\end{lstlisting}

